Robust Control for Signal Temporal Logic Specifications using Average Space Robustness

Control systems that satisfy temporal logic specifications have become increasingly popular due to their applicability to robotic systems. Existing control methods, however, are computationally demanding, especially when the problem size becomes too large. In this paper, a robust and computationally efficient model predictive control framework for signal temporal logic specifications is proposed. We introduce discrete average space robustness, a novel quantitative semantic for signal temporal logic, that is directly incorporated into the cost function of the model predictive controller. The optimization problem entailed in this framework can be written as a convex quadratic program when no disjunctions are considered and results in a robust satisfaction of the specification. Furthermore, we define the predicate robustness degree as a new robustness notion. Simulations of a multi-agent system subject to complex specifications demonstrate the efficacy of the proposed method.

==> chapter/case_study.tex <==
\section{Case Study}
\label{sec:case_study}
\re{Under construction/will be removed}
The system under consideration is the coupled two-tank process introduced in Section \ref{sec:robustness_notions}. However, we now consider additive noise $\boldsymbol{v}(k)$ as
\begin{align}
\boldsymbol{x}(k+1) = \begin{bmatrix}
0.79 & 0\\
0.176 & 0.0296
\end{bmatrix}\boldsymbol{x}(k)+
\begin{bmatrix}
0.281\\
0.0296
\end{bmatrix}\boldsymbol{u}(k)+ \boldsymbol{v}(k)
\end{align}
with $\boldsymbol{u}(k) \in [0,6]$ and the formulas
\begin{align*}
\phi_1&=event \implies F_{[ 120,240 ]} (x_1\ge2) \\
\phi_2&=G_{[ 0,\infty ]}\big((x_1\ge0) \until{120}{240} (x_1\le5)\big)\\
\phi_3&=G_{[ 0,\infty ]} \big(F_{[120,240]}(x_1\ge2) \wedge \\ 
& \hspace{3cm} (x_1\le4) \until{180}{420} (x_2\le2.5)\big).
\end{align*}
The noise level is indicated by the Signal-to-Noise ratio as $\text{SNR}_{\text{dB}} = 10 \cdot \operatorname{log}_{10}\Bigl(\frac{P_{\boldsymbol{x}}}{P_{\boldsymbol{v}}}\Bigr)$, where $P_{\boldsymbol{x}}$ denotes the average signal power. For the simulations of this section we set $M=\underline{0}_{m,m}$, i.e., no input minimization is considered.


Fig. \ref{fig:1} shows $\phi_1=event \implies F_{[120,240]} (x_1\ge2)$, where $event$ is triggered at $120$ seconds, i.e., $k_{event}=\kl 120,120 \kr$. Note that Fig. \ref{fig:MPC_oneshots_eve_inf} displays the case without any noise, while Fig \ref{fig:MPC_oneshots_eve_11.76} indicates the case where noise is present. However, in both cases the algorithm starts increasing the water level $x_1$ at $t=120$ seconds to its maximum at $t=360$ seconds; $\phi_2=G_{[ 0,\infty ]}\big((x_1\ge0) \until{120}{240} (x_1\le5)\big)$ is an all-time satisfying formula and displayed in Fig. \ref{fig:2} with and without noise. The minima of $x_1$ correspond to the times where $x_1\le5$ is minimized, while in between these points $x_1\ge 0$ is maximized. Finally, Fig. \ref{fig:3} shows $\phi_3=G_{[ 0,\infty ]}\big(F_{[120,240]}(x_1\ge2) \wedge (x_1\le4) \until{180}{420} (x_2\le2.5)\big)$. Maxima in $x_1$ correspond to maximizing $x_1\ge2$, whereas minima in $x_2$ indicate minimizing $x_2\le2.5$. Note that the algorithm always tries to minimize $x_1\le 4$. Finally note that all formulas $\phi_1$, $\phi_2$, and $\phi_3$ are satisfied by the proposed control strategy, with and without noise.

\begin{figure*}
\centering
\begin{subfigure}{0.48\textwidth}\caption{$\text{SNR}_{\text{dB}}=\infty$}\label{fig:MPC_oneshots_eve_inf}
\input{figures/MPC_oneshots_eve_inf}
\end{subfigure}
\begin{subfigure}{0.48\textwidth}\caption{$\text{SNR}_{\text{dB}}=10.8625$}\label{fig:MPC_oneshots_eve_11.76}
\input{figures/MPC_oneshots_eve_11.76}
\end{subfigure}
\caption{$\phi_1= event \implies F_{[ 120,240 ]} (x_1\ge2)$}
\label{fig:1}
\end{figure*}


\begin{figure*}
\centering
\begin{subfigure}{0.48\textwidth}\caption{$\text{SNR}_{\text{dB}}=\infty$}\label{fig:mpc_until_inf}
\input{figures/mpc_until_inf}
\end{subfigure}
\begin{subfigure}{0.48\textwidth}\caption{$\text{SNR}_{\text{dB}}=13.6128$}\label{fig:mpc_until_13.5035}
\input{figures/mpc_until_13.5035}
\end{subfigure}
\caption{$\phi_2=G_{[ 0,\infty ]}\big((x_1\ge0) \until{120}{240} (x_1\le5)\big)$}
\label{fig:2}
\end{figure*}

\begin{figure*}
\centering
\begin{subfigure}{0.48\textwidth}\caption{$\text{SNR}_{\text{dB}}=\infty$}\label{fig:mpc_coneveuntil_inf}
\input{figures/mpc_coneveuntil_inf}
\end{subfigure}
\begin{subfigure}{0.48\textwidth}\caption{$\text{SNR}_{\text{dB}}=11.2937$}\label{fig:mpc_coneveuntil_10.4075}
\input{figures/mpc_coneveuntil_10.4075}
\end{subfigure}
\caption{$\phi_3=G_{[ 0,\infty ]}\big(F_{[120,240]}(x_1\ge2) \wedge (x_1\le4) \until{180}{420} (x_2\le2.5)\big)$}
\label{fig:3}
\end{figure*}


The SNR for these examples ranges from $10.8625$ to $13.6128$ dB and satisfaction is still ensured due to the robust receding horizon implementation. The MPC implementation steers the state trajectory in the direction away from the set of states not fulfilling the formula. As it was indicated in Section \ref{sec:robustness_notions}, maximizing DSASR increases the predicate robustness degree. Note that the mixed integer linear programs in \cite{raman1,raman2,sadraddini} are computationally demanding and increase the robustness degree only if SR is included in the cost function. This makes the optimization problem inherently nonconvex. Our implementation makes sure that the robustness degree is positive while maximizing the predicate robustness degree. In other words, the formula is satisfied while the predicate robustness degree is maximized.

%The difference of DSASR and SR can also be discussed by having a look at the until-operator $(x_1\le4) \until{180}{420} (x_2\le2.5)$ in contained in $\phi_3$ and displayed in Fig. \ref{fig:3}. The algorithm, using DSASR, tries to maximize $x_1\le 4$ all the time due to the average approach. SR as in Definition \ref{def:2} would not necessarily do the same and only try to elevate the satisfaction of the weakest point. For example, depending on the situation SR would rather try to maximize $x_1\ge 5$ instead of $x_1\le 4$, whereas DSASR will maximize satisfaction of $x_1\ge 5$ and $x_1\le 4$ at the same time since a weighted average of them is used in their definition. \re{this might need some treatment}
 




